SDSS-IV MaNGA: A Catalogue of Spectroscopically Detected Strong Galaxy-Galaxy Lens Candidates

We spectroscopically detected candidate emission-lines of 8 likely, 17 probable, and 69 possible strong galaxy-galaxy gravitational lens candidates found within the spectra of ~10,000 galaxy targets contained within the completed Mapping of Nearby Galaxies at Apache Point Observatory (MaNGA) survey. This search is based upon the methodology of the Spectroscopic Identification of Lensing Objects (SILO) project, which extends the spectroscopic detection methods of the BOSS Emission-Line Lensing Survey (BELLS) and the Sloan Lens ACS Survey (SLACS). We scanned the co-added residuals that we constructed from stacks of foreground subtracted row-stacked-spectra (RSS) so a sigma-clipping method can be used to reject cosmic-rays and other forms of transients that impact only a small fraction of the combined exposures. We also constructed narrow-band images from the signal-to-noise of the co-added residuals to observe signs of lensed source images. We also use several methods to compute the probable strong lensing regime for each candidate lens to determine which candidate background galaxies may reside sufficiently near the galaxy centre for strong lensing to occur. We present the spectroscopic redshifts within a value-added catalogue (VAC) for data release 17 (DR17) of SDSS-IV. We also present the lens candidates, spectroscopic data, and narrow-band images within a VAC for DR17. High resolution follow-up imaging of these lens candidates are expected to yield a sample of confirmed grade-A lenses with sufficient angular size to probe possible discrepancies between the mass derived from a best-fitting lens model, and the dynamical mass derived from the observed stellar velocities.

==> notes/dr17+/silo_vac_update-20220608.tex <==
Spectroscopic Redshifts for MaNGA Spectra

Our catalog contains precise spectroscopic redshifts (M. Talbot et al. in prep.) for spaxels and RSS in MaNGA. This catalog is an update to an earlier version released in Talbot et al. 2018 but instead includes the entire sample of galaxies from the completed MaNGA survey. In brief, our software uses the spec1d – zfind code to compute the spectroscopic redshifts, which zfind is available from the publicly accessible BOSS pipeline~\citep{2012AJ....144..144B}. The zfind code requires an initial redshift guess obtained from the NSA catalog in the first pass. A second pass uses the mean spectroscopic redshift within the high signal-to-noise region of the target as the initial guess for zfind to successfully compute spectroscopic redshifts for low signal-to-noise spectra that a redshift could not be determined in the first pass. Successful computations of the spectroscopic redshift and fitted foreground model are contained in this VAC.

Strong Gravitational Lens Candidates Found in MaNGA

This VAC contains eight likely, 17 probable, and 69 possible strong galaxy-galaxy scale gravitational lens candidates we discovered in the final release of the MaNGA survey. These candidates are found by the Spectroscopic Identification of Lensing Object project~\citep[SILO;][M. Talbot et al. in prep]{2018MNRAS.477..195T}, which search method adds to the BELLS~\citep{2012ApJ...744...41B} spectroscopic detection method to identify emission-lines of background galaxies within spectra. We scanned residuals computed from co-adding foreground-subtracted RSS across exposures from the same fiber and dither position. The quality of each background emission-line, its proximity to a projection of the probable strong lensing regime, and the presence of lensing features within narrowband images constructed from the signal-to-noise of the co-added residuals are primarily considered in assigning a candidate likelihood grade to each candidate. Since the first announcement of this VAC in DR17~\citep{2022ApJS..259...35A}, we added more kinematic and image quality filters to improve the accuracy and computation success of the probable strong lensing regime. Detection information, narrowband image data, computations of the probable strong lensing regime, inspection information, Gaussian fits of the candidate emission-lines, and quick-view spectra and narrowband plots of the detection are presented in this VAC.



==> notes/michaelreponse_20220531.tex <==
I thank the authors who have provided answers to my comments and have improved the readability of the paper, adding more text, more figures, more analyses. However, before the paper can be accepted for publication I have a few more comments that the authors would address. Note that  I read the version including the green edits, so I will refer to pages and positions related to that manuscript version.

MAIN COMMENTS

- Unfortunately the authors provided to me a version with edits (the one with green text) which presents some issues. I have discovered this only during the latest stages of my report, since I was using this version as reference. I see that the submitted version without edits and the one with edits totally differ on the sectioning of section 2, since in the version with the edits the section on "Narrow-band SN..." was not there. A similar issue is present in section 3.3 where for example the text "The distribution of the JAM...." is missing in the version I have referred (I have not checked if there were other mismatches among the two versions). Please, the next time send the version which include edits, but do double checks, using the proper version, since this could complicate my report.  During the update of a manuscript after a referee report is always important take note of the updates directly on the manuscript to facilitate the work of the referee, who can decide to read all the paper again but also focus only on the changes, if he/she believe that the rest of the paper does not need further changes.
>Thank you for spotting this. Somehow these missing text were accidentally removed in the final stages of edits to the highlighted version. Both are now fixed.

- There is yet a long list of typos, that I quoted in the list at the end of the report.
>See fixes in list you mentioned.

- On the new introduction. I thank the authors to have included a lot of information, which is very useful for the reader, but now the size of the introduction is very large, almost five columns, 2 pages and half. This is just a suggestion, can probably be  more useful to remove some piece from the intro and create a new Section 2, including some of the new text the authors have now included, e.g. the one on the future scientific outcomes of this search? The section could  be named something like "Aims and objectives"? Then, the description of the galaxy sample could also be moved to the section now named "Spectroscopic Selection", that can be re-named as "Sample and spectroscopic selection" or something similar.
>We moved MaNGA sampling and objectives to two new sections and minimized re-explaining data such as RSS and the uses of MaNGA data in the introduction.

- Just a general comment on the total mass density slope, also if not relevant for the analysis of the paper. The trend with mass confirms to me that the sample is full of late-type systems. In fact while late-type systems present the trend with mass you are finding,  confirming Li+19 results, early-types (which would populate the more massive side) would do the opposite, with steeper slopes at lower masses.
>Nice comment.

Typo/minor comments

- In the abstract, "to probe discrepancies" -> "to probe possible discrepancies"?
>Done

- Add a comma after "Thomas" in the list of authors
>Done

- Page 2, "a number biases" -> "a number of biases"?
>Done

"fsample" -> "sample"?
>Issue in highlighted version is fixed. Issue not in non-highlighted version you read, which we now use to highlight changes in this pass. 

- Page 3, what do the authors mean with "to reside within arcseconds of \approx 10'' targets"?
>Re-wrote as replacement '...to be approximately the physical size of the bulge for MaNGA targets...', which simplifies our attempt to contrast arcsecond-scale strong lensing regime vs ~10" visible region of galaxy.

- Page 4, bullets in section 4, do the authors think that adding some bold text at the beginning of each bullet can help? I mean, in the bullet starting with "Model and remove...", they can start with "{\bf Foreground Galaxy subtration}", which is also the title of the related subsection where they are providing more details on this item....and the same for the other ones. This is just a suggestion....
>Added first suggestion to first bullet and '{\bf Search for remaining background signals.}' to the second bullet.

- Page 4, in the bullet "Scan fpr sets..." mention subsection 2.3
>Done. Sentence now starts with 'Scan for sets of high SN signals within the co-added residuals (see Section 2.3)...'

- Page 4, on the bullet "Narrow-band....", to what section is this referring to? I do not find it...see the next point, there is an error referring to the section..... (ok, this is the issue I was mentioning at the beginning of the report)
>Automatically fixed by restoring the missing text you referred too.

- Page 4, fix "Section ?? describes" (left column) and "(see Section ??)" (right column).
>Automatically fixed by restoring the missing text you referred too.

- Page 4, left column, "(see Section 2.2." missing parenthesis
>Fixed

- Page 4, "galaxy spectra templates" -> "galaxy spectral templates"?
>Done

- Page 4, left, is this sentence correct? "...flux patterns of expected background emissions, which the latter includes..."
>The related sentence is now broken into several sentences and further modified to increase verbosity and specify order of processes.

- Page 4, right column, fix this sentence "of the signal across the narrow-band image and the detections demonstrate; lensing features"
>Removed ' across the narrow-band image and the detections ' as this was redundent. Also added 's' to 'demonstrate' as spotted by Grammarly.

- Page 4, please, at the end of the first part of section 4, or somewhere around there, clearly mention that in the following section each item/bullet will be detailed....
>Added before Section 2.1 'In the following sections, we describe each stage of these mentioned methods.'

- Page 9, please do this sentence "...can induce a bias in spaxels, which affected regions are often related.." need to be fixed?
>Replaced ', which' with '. These'

- Page 10, "(see Figure 1 and 3)" -> "(see Figures 1 and 3)"
>Done

- Page 10, section 3.2, it could help to do this update: "likely" -> "likely (Grade A)", and similarly for "probable" and "possibly".
>Done for first time mentioned in results section

- Page 10, section 3.3, fix the sentence, "Figure 4 demonstrates.....", 
>We reduced information that was reduntant to future explanations, enabling this sentence to be re-written to 'Figure 4 demonstrates that fitted JAM kinematic projections of MaNGA target SDSS J1344+2620 approximate the DAP kinematic measurements used in the fit.'

and also "Inspection of kinematic maps reveal failure to fit JAM to  the remaining quarter of the targets with candidate background galaxies is primarily caused by poorer kinematic measurements of fainter  and low-mass galaxies failing to pass masking and fitting processes described in Section B.", for example, a "which" is missing before "is primarily"?
>We broke the sentence into two and added a few modifiers. The sentence now reads 'Inspection of kinematic maps reveals JAM fails to fit the remaining quarter of targets with candidate background galaxies. This issue is primarily caused by poorer kinematic measurements of fainter and low-mass galaxies failing to pass masking and fitting processes described in Section 4.'

- Page 10, please, when quoting appendices use "Appendix" and not "Section" (also in the rest of the paper). left column, "Sections 2.5.2 and B1", add "Appendix" before "B1",
>Changed related 'Section' to 'Appendix'


-"Dutton & Macciò (2014); Girelli et al. (2020)" -> "(Dutton & Macciò 2014, Girelli et al. 2020)"? 
>Done

- And is "which relations are..." correct sentence? is 
>We put a period before 'which' and re-wrote latter half as this 'Thus the scaling between the stellar mass and the dark matter halo is fixed in the JAM modeling process and demonstrate no scatter.'

-"with approximately an effective radius" correct form in "...yield relatively small uncertainties with approximately an effective radius"?, 
>Now reads: This stellar to dark matter scaling is desirable since MaNGA kinematic measurements are only well constrained within approximately an effective radius ($R_{eff}$) of the target, which is insufficient for a fit to isolate the low dark matter fraction within this region.


"Treu et al. (2006); Bolton et al. (2012b); Li et al. (2018a)." -> "(Treu et al. 2006, Bolton et al. 2012b, Li et al. 2018a)."
>Fixed

- Page 10, right column, I guess that "Reff = 0.1" and "Reff = 1" mean "R/Reff = 0.1" and "R/Reff=1"? Please, fix it.
>Fixed

- Please, write clearly in the text that figure 3,5 and 6 just put together the results for all the galaxies, analyzed independently.  This kinds of plots can confuse the reader, since it is typically used to show the results of likelihood maximization.
>Added to first paragraph in results: 'All corner plots represent distributions of fitted model parameters across samples specified in the following sections or figure captions.'

- Figure 4, at this point, show 3 panels, the third with residuals, if possible.
>>>Joel, this and some other plot edit suggestions will need access from the SILO databases we migrated.

- Page 12, left column, "Talbot et al. (2018)" -> "(Talbot et al. 2018)"
>Done

- Figure 6, please, fix the symbol for stellar mass in the appendix. Is "The demonstrated stellar mass is the..." correct? 

- What is "LER" in the panels? 
>Added to Figure 6: 'The ratio between the lower limit of the Einstein radii projections (LER) and the upper limit tends to increase with mass.'

- and also fix the symbols for M^star_\odot in the panels....
>>>

- Page 14, is the sentence "...solar masses are present in all grades, but the lowest mass is;..." correct?
>We broke this sentence at the comma and removed 'but'.

- Page 16, "are on the order"? Is "are of the order" more correct? And "(see Figure 4 of Brownstein et al. (2012))" -> "(see Figure 4 of Brownstein et al. 2012)", "Smith et al. (2020)" -> "(Smith et al. 2020)"
>Did all suggestions.

- Caption of figure 8, please, specify that these are among the best candiates.
>Added '(Grade A- or above)' after 'likely' in first sentence.

- Appendix A, please, fix the fit of the table in the page.
>It looks like Table A1 is the issue since the rotated caption overlaps with other page information. Thus I reduce the caption width.

- At page 29, appendix B3, the authors mention the "elliptical radius (Re)", what is it?
>Added a bit more verbosity. That sentence has been expanded into the following: '...SILO first computes an elliptical radius Re with a major to minor axis ratio and position angle that approximates contours of constant $\sigma_{LOS}$ within the $\sigma_{LOS}$ map of the target. The Re is approximated using the PA measurement and the major to minor axis ratio of the SDSS Sersic fit of the target...'

- Page 30, "determening" -> "determining"
>Done

----------------------------------------------
MT: Noted following sufficiently warrented stated change.
Page 2: If improvements in dynamical modelling do not resolve the lens-dynamic mass discrepancy, then the discrepancy can be compared between low and high redshift lenses to infer LOS \strikedtext{density}\addedtext{influences}.

Figure 6: changed 219 to 212

==> tex/tables/apdx_vac_lens_stack_1.dat.tex <==
AUTHOR & String & Creator of detection file  \\
INSP & String & Detection inspector  \\
SOURCE & String & SILO  \\
SILO\_VER & String & Version build of SILO  \\
DRPVER & String & Data reduction pipeline version of RSS spectra  \\
SAMPLING & String & Wavelength sampling type  \\
SPECTRA & String & Type of spectra used from MaNGA files  \\
OBJRA\textsuperscript{a} & Float & Object right ascension  \\
IFURA\textsuperscript{a} & Float & Right ascension of IFU center  \\
OBJDEC\textsuperscript{a} & Float & Object declination  \\
IFUDEC\textsuperscript{a} & Float & Declination of IFU center  \\

==> tex/tables/apdx_vac_lens_stack_2.dat.tex <==
RSS\_INDEX & Integer & Row-stacked spectra index  \\
DITHER\_POSITION & String & Fiber position in dither pattern  \\
FIBER\_INDEX & Integer & Fiber index within IFU  \\
FIBER\_POSITION & String & Fiber number in IFU and dither position  \\
EXPNUM & Integer & Exposure number  \\
SET & Integer & Iteration of dither pattern set  \\
SEEING\textsuperscript{a} & Float & Seeing at time of exposure  \\
MEAN\_X\textsuperscript{a} & Float & Mean x position of fiber  \\
MEAN\_Y\textsuperscript{a} & Float & Mean x position of fiber  \\
MEAN\_R\textsuperscript{a} & Float & Mean radius position of fiber  \\
SPECZ & Float & Best fit redshfit of spectra in fiber  \\
FLUX\textsuperscript{b} & Float (Array) & Flux of spectra  \\
IVAR & Float (Array) & Inverse variance of spectra  \\
MASK & Integer (Array) & Bit mask of spectra  \\
XPOS\textsuperscript{a} & Float (Array) & X position of wavelenth-dependent spectra  \\
YPOS\textsuperscript{a} & Float (Array) & Y position of wavelenth-dependent spectra  \\
RPOS\textsuperscript{a} & Float (Array) & Radius of wavelenth-dependent spectra  \\
MODEL\textsuperscript{b} & Float (Array) & SILO model of flux  \\
RESFLUX\textsuperscript{b} & Float (Array) & Residual spectra of flux-model  \\
IVAR\_RES & Float (Array) & Rescaled inverse variance of residual spectra  \\
SN\_SPEC & Float (Array) & Gaussian convolved SN of residual spectra  \\
O2SN\_SPEC & Float (Array) & OII Gaussian convolved SN of residual spectra  \\
